Factorization Algebras for Bulk-Boundary Systems

Costello and Gwilliam have given both 1) a general definition of perturbative quantum gauge theory on a manifold M and 2) a construction of a factorization algebra of quantum observables assigned to every quantum gauge theory. In this dissertation, we extend these constructions to a certain general class of field theories on manifolds with boundary.

==> Chapters/PropagatorProof.tex <==
Let us consider the asymptotic expansion of the heat kernel:
\begin{equation}
    \tilde K_L \simeq L^{-n/2}e^{-||x-y||^2/(4L)}\sum_{i \geq 0}L^i \Omega_i(x,y),
\end{equation}
where the $\Omega_i$ are smooth sections of $\Edbl\boxtimes \Edbl$.
We would like to define
\begin{equation}
\label{eq: defofTL}
    T_L e = \lim_{\epsilon\to 0} \int_\epsilon^L \id \otimes \ip \left( K_{T}|_{M\times M} \otimes e\right)\d T.
\end{equation}
As discussed above, we may view $e$ as a distributional section of $\Edbl$on $\Mdbl$, simply by extending it by zero on the negative half-manifold.
The resulting section has singular support on $\bdyM$.
The limit defining $T_L$ exists for $e\in \sEdbl$ and defines a pseudodifferential operator on $\sEdbl$.
Hence, $T_L e$ exists as a distributional section of $\Edbl$.
Because $T_L$ is a pseudo-differential operator, it preserves the singular support of sections; hence, we may understand $T_Le$ as a distributional section of $\Edbl$ which is smooth away from $\bdyM\subset \Mdbl$.
Let us denote by $g$ the smooth section of $E\to \mathring M$ produced in this way.
By the Seeley extension theorem, it suffices to show that $g$ has bounded derivatives of all orders on $\mathring M$; then $g$ will extend to a smooth section of $E$ over all of $M$.
If we bound these derivatives in a way which is uniform in the $C^k$ norms of $e$, we will show that the limit defining $T_L$ exists as a continuous map $\condfieldscs\to \sE_c$.
Because of the $\involution$-invariance of the heat kernel, and because $(\ultrafields)_c$ and $\condfieldscs$ are closed subsets of $\sE_c$, $T_L$ will factor through the map
\begin{equation}
    (\ultrafields)_c \to \condfieldscs \to \sE_c.
\end{equation}

Since the singularities of $T_L$ are on the diagonal, this is a purely local question and we may replace $K_{L}$ with its asymptotic expansion.
The propagator $P(\Phi_L)$ will be obtained from $\Phi_L$ by the application of derivatives to the kernel.
Hence, given a multi-index $\alpha\in \NN^n$, we would like to study the following integral:
\begin{align}
    &g(x):=\nonumber\\
    &\lim_{\epsilon \to 0}\int_\epsilon^L \frac{1}{T^{n/2-i+|\alpha|}} \int_{\HH^n}\left((y-x)^\alpha e^{-\frac{||x-y||^2}{4T}}\Omega_i (x,y)\pm (y-x^*)^\alpha e^{-\frac{||y-x^*||^2}{4T}}\Omega_i (x^*,y)\right) f(y) \d^n y\d T.
\end{align}
Here, $\Omega_i$ is a properly supported smooth function on $\RR^n\times \RR^n$, $f$ is a compactly-supported smooth function on $\HH^n$, and 
\begin{equation}
(y-x)^\alpha = (y_1-x_1)^{\alpha_1}\cdots (y_n-x_n)^{\alpha_n}.
\end{equation}
We note that, at most, $\alpha_n=1$, since we have prescribed that $Q^{GF}$ involves only one derivative in the normal direction.
We would like to show:
\begin{enumerate}
    \item The limit defining $g$ exists.
    \item The norm $|g(x)|$ can be bounded globally bounded as $x\in \HH^n$ by bounding the $C^k$ norms of $f$.
    \item All derivatives of $g$ exist.
    \item All derivatives of $g$ are bounded on the interior $\mathring \HH^n$.
\end{enumerate}
To this end, let us write $y=(\dot y, y_n)$ for the decomposition of $y$ with respect to the isomorphism $\HH^n\cong \RR^{n-1}\times \RR_{\geq 0}$.
We will similarly write $\alpha = (\dot \alpha, \alpha_n)$.
Note that
\begin{equation}
    \frac{(\dot y - \dot x)^{\dot \alpha}}{T^{|\dot \alpha|}}e^{-\frac{||x-y||^2}{4T}}= (-2)^{|\dot \alpha|}\left( \frac{\del}{\del y_1}\right)^{\alpha_1}\cdots \left( \frac{\del}{\del y_{n-1}}\right)^{\alpha_{n-1}}e^{-\frac{||x-y||^2}{4T}}=:D_y^{\dot \alpha}e^{-\frac{||x-y||^2}{4T}}
\end{equation}
We may therefore integrate by parts, and we find that 
\begin{align}
    g(x):=&-\lim_{\epsilon \to 0}\int_\epsilon^L \frac{1}{T^{n/2-i+\alpha_n}} \int_{\HH^n}(y_n-x_n)^{\alpha_n}e^{-\frac{||x-y||^2}{4T}}D_y^{\dot \alpha}\left(\Omega_i (x,y)f(y)\right)\d^n y\, \d T\nonumber\\
    &\mp\lim_{\epsilon \to 0}\int_\epsilon^L \frac{1}{T^{n/2-i+\alpha_n}} \int_{\HH^n}(y_n+x_n)^{\alpha_n}e^{-\frac{||y-x^*||^2}{4T}}D_y^{\dot \alpha}\left(\Omega_i (x^*,y) f(y) \right)\d^n y\,\d T.
\end{align}

The functions $\Omega_i(x,y)f(y)$, $\Omega_i(x^\star, y)f(y)$---as functions on $\RR^n\times \HH^n$---have compact support.
Therefore, so too do all their derivatives.
Set
\begin{equation}
    \Omega_{i,\dot \alpha, f}(x,y) = D^{\dot \alpha}_y \left(\Omega_{i}(x,y) f(y)\right)
\end{equation}
Let us change coordinates, setting $y'=y-x$ or $y'=y-x^*$.
Thus, we find that 
\begin{align}
    g(x)&=\nonumber\\
   - & \lim_{\epsilon\to 0}\int_\epsilon^L \frac{1}{T^{n/2-i+\alpha_n}}\int_{\RR^{n-1}}\int_{-x_n}^\infty (y'_n)^{\alpha_n} e^{-\frac{||y'||^2}{4T}} \Omega_{i,\dot \alpha,f}(x,y'+x)\d y'_n \,\d^{n-1}\dot y' \,\d T\nonumber\\
    \mp&\lim_{\epsilon\to 0}\int_\epsilon^L \frac{1}{T^{n/2-i+\alpha_n}}\int_{\RR^{n-1}}\int_{x_n}^\infty (y'_n)^{\alpha_n} e^{-\frac{||y'||^2}{4T}}\Omega_{i,\dot \alpha,f}(x^*,y'+x^*)\d y'_n\, \d^{n-1} \dot y'\, \d T.
    \label{eq: changedcoordsGaussianintegral}
\end{align}
Let $M(i,\dot \alpha,f)$ denote the maximum value of $|\Omega_{i,\dot \alpha,f}|$.
$M(i,\dot \alpha,f)$ is bounded by a polynomial in the $C^k$ norms of $f$.
We find that
\begin{align}
    |g(x)|&\leq \nonumber\\
    &M(i,\dot \alpha,f) \lim_{\epsilon\to 0}\int_\epsilon^L \frac{1}{T^{n/2-i+\alpha_n}}\int_{\RR^{n-1}}\int_{-\infty}^\infty |y'_n|^{\alpha_n} e^{-\frac{||y'||^2}{4T}} \d y'_n \,\d^{n-1}\dot y' \,\d T\nonumber\\
    +&M(i,\dot \alpha, f)\lim_{\epsilon\to 0}\int_\epsilon^L \frac{1}{T^{n/2-i+\alpha_n}}\int_{\RR^{n-1}}\int_{-\infty}^\infty |y'_n|^{\alpha_n} e^{-\frac{||y'||^2}{4T}}\d y'_n\, \d^{n-1} \dot y'\, \d T.
\end{align}
Upon performing the Gaussian integral, we obtain a bound for $|g(x)|$.
Now, we need to show that the derivatives of $g$ are bounded.
To this end, Equation \eqref{eq: changedcoordsGaussianintegral} proves useful.
We note that any derivative of $g$ along $\RR^{n-1}$ can be described by a similar integral to the one defining $g$, but with $\Omega_{i,\dot \alpha, f}$ replaced by its corresponding derivative.
Hence any derivative of $g$ along $\RR^{n-1}$ can be shown to be bounded by the same reasoning as above.
For fixed $x_n>0$, taking the derivative with respect $x_n$ will also produce such a term, but will also introduce the following quantity:
\begin{align}
    g_n(x):&=\nonumber\\
   & \lim_{\epsilon\to 0}\int_\epsilon^L \frac{1}{T^{n/2-i+\alpha_n}}\int_{\RR^{n-1}} (-x_n)^{\alpha_n} e^{-\frac{||\dot y||^2+x_n^2}{4T}} \Omega_{i,\dot \alpha,f}(x,(\dot y'+\dot x,0)) \,\d^{n-1}\dot y' \,\d T\nonumber\\
    \pm&\lim_{\epsilon\to 0}\int_\epsilon^L \frac{1}{T^{n/2-i+\alpha_n}}\int_{\RR^{n-1}} (x_n)^{\alpha_n} e^{-\frac{||\dot y'||^2+x_n^2}{4T}}\Omega_{i,\dot \alpha,f}(x^*,(\dot y'+\dot x,0)) \d^{n-1} \dot y'\, \d T.
\end{align}
For $x_n>0$, the integrand for the integral defining $g_n(x)$ is compactly-supported and smooth in $(x,\dot y',T)\in \HH^n\times \RR^{n-1}\times [0,L]$.
Hence, we may simply integrate over $[0,L]$ without taking a limit.
We may also bring derivatives with respect to $x_n$ into the integral.
We find:
\begin{align}
   &\frac{\del^k g_n(x)}{(\del x_n)^k}=\nonumber\\
   & C\int_0^L \frac{1}{T^{n/2-i}}\int_{\RR^{n-1}}  e^{-\frac{||\dot y||^2}{4T}} \left(\frac{\del}{\del x_n}\right)^{\alpha_n+k}\left(e^{-\frac{x_n^2}{4T}}\Omega_{i,\dot \alpha,f}(x,(\dot y'+\dot x,0))\right) \,\d^{n-1}\dot y' \,\d T.\nonumber\\
\end{align}
It therefore suffices to consider the boundedness in $x_n$ of the following quantity, where $\Upsilon(x,\dot y')$ is a compactly-supported smooth function on $\HH^n\times \RR^{n-1}$:
\begin{align}
    &g^{k'}(x):=\nonumber\\
    &\int_{0}^L \left(\frac{\del}{\del x_n}\right)^{k'}\left(e^{-\frac{x_n^2}{4T}}\right) \frac{1}{T^{n/2-i}}\int_{\RR^{n-1}} e^{-\frac{||\dot y||^2}{4T}} \Upsilon(x,\dot y') \d^{n-1}\dot y'\, \d T.
\end{align}
Let us perform the Taylor expansion of $\Upsilon$ in the $\dot y'$ variables:
\begin{equation}
    \Upsilon(x,\dot y') = \sum_{|\alpha|< N} (\dot y')^\alpha \left(\frac{\del}{\del \dot y'}\right)^{\alpha}\Upsilon(x, 0)+\sum_{|\alpha| = N} (\dot y')^\alpha R_{N,\alpha}(x,\dot y').
\end{equation}
Hence,
\begin{align}
    &g^{k'}(x)=\nonumber\\
    &\sum_{|\alpha|<N}C_\alpha \left(\frac{\del}{\del \dot y'}\right)^{\alpha}\Upsilon(x, 0)\int_0^L \left(\frac{\del}{\del x_n}\right)^{k'}\left(e^{-\frac{x_n^2}{4T}}\right) \frac{1}{T^{1/2-i-|\alpha|/2}} \d T\nonumber\\
    &+ \sum_{|\alpha|=N} \int_{0}^L \left(\frac{\del}{\del x_n}\right)^{k'}\left(e^{-\frac{x_n^2}{4T}}\right) \frac{1}{T^{n/2-i}}\int_{\RR^{n-1}} e^{-\frac{||\dot y||^2}{4T}} (\dot y')^\alpha R_{N,\alpha}(x,\dot y')\d^{n-1}\dot y'\, \d T.
\end{align}
The $k'$-th derivative of $e^{-x_n^2/(4T)}$ is a polynomial in $1/T$.
We may therefore choose $N$ large and bound $R_{N,\alpha}$ by a quantity depending only on the $C^k$ norms of $\Upsilon$.
This will guarantee that no negative powers of $T$ appear in the $T$ integral, except in the exponential $e^{-x_n^2/4T}$.
Such integrals are manifestly seen to be bounded.
It therefore suffices to check the boundedness of the quantities
\begin{equation}
    \int_0^L \left(\frac{\d}{\d x_n}\right)^{k'}\left(e^{-\frac{x_n^2}{4T}}\right) \frac{1}{T^{1/2-i-|\alpha|/2}} \d T = \left(\frac{\d}{\d x_n}\right)^{k'}\int_0^L e^{-\frac{x_n^2}{4T}} \frac{1}{T^{1/2-i-|\alpha|/2}} \d T
    \label{eq: pregammaint}
\end{equation}
The integral on the right-hand side of Equation \eqref{eq: pregammaint} gives
\begin{equation}
    C (x_n^2)^{1/2+i+|\alpha|/2} \Gamma\left(1/2+i+|\alpha|/2, \frac{x_n^2}{4L}\right),
\end{equation}
which is manifestly bounded and has bounded derivatives in $x_n$.
This completes the proof.
